Amnesic Probing: Behavioral Explanation with Amnesic Counterfactuals

A growing body of work makes use of probing to investigate the working of neural models, often considered black boxes. Recently, an ongoing debate emerged surrounding the limitations of the probing paradigm. In this work, we point out the inability to infer behavioral conclusions from probing results and offer an alternative method that focuses on how the information is being used, rather than on what information is encoded. Our method, Amnesic Probing, follows the intuition that the utility of a property for a given task can be assessed by measuring the influence of a causal intervention that removes it from the representation. Equipped with this new analysis tool, we can ask questions that were not possible before, e.g. is part-of-speech information important for word prediction? We perform a series of analyses on BERT to answer these types of questions. Our findings demonstrate that conventional probing performance is not correlated to task importance, and we call for increased scrutiny of claims that draw behavioral or causal conclusions from probing results.

==> figures/layer_wise_deprobe.tex <==

\begin{figure*}[ht!]
\centering
\subfloat{
\includegraphics[width=0.235\textwidth]{figures/layer_wise_deprobe_tag_normal.pdf}
}
\subfloat{
\includegraphics[width=0.235\textwidth]{figures/layer_wise_deprobe_ner_normal.pdf}
}
\subfloat{
\includegraphics[width=0.235\textwidth]{figures/layer_wise_deprobe_phrase_start_normal.pdf}
}
\subfloat{
\includegraphics[width=0.235\textwidth]{figures/layer_wise_deprobe_phrase_end_normal.pdf}
} \\

\subfloat{
\includegraphics[width=0.235\textwidth]{figures/layer_wise_deprobe_tag_masked.pdf}
}
\subfloat{
\includegraphics[width=0.235\textwidth]{figures/layer_wise_deprobe_ner_masked.pdf}
}
\subfloat{
\includegraphics[width=0.235\textwidth]{figures/layer_wise_deprobe_phrase_start_masked.pdf}
}
\subfloat{
\includegraphics[width=0.235\textwidth]{figures/layer_wise_deprobe_phrase_end_masked.pdf}
}

\caption{Layer-wise removal. Removing from layer i (the rows) and testing performance on layer j (the columns). First row is unmasked version, second is masked.}
\label{fig:layer_wise_removal_probe}
\end{figure*}


==> tables/layer_tag_lm.tex <==
\begin{table}[th]
\centering
\resizebox{\columnwidth}{!}{%

\begin{tabular}{r|r|rrr}
\toprule
 layer &  probing &  rand dir lm &  task &  -P lm \\
\midrule
     0 &    83.65 &        94.53 &           83.28 &  82.44 \\
     1 &    92.81 &        93.25 &           90.02 &  95.11 \\
     2 &    94.16 &        92.87 &           89.97 &  96.38 \\
     3 &    95.09 &        94.27 &           88.45 &  94.65 \\
     4 &    95.88 &        91.63 &           86.47 &  89.54 \\
     5 &    95.91 &        91.86 &           72.44 &  74.87 \\
     6 &    95.90 &        93.37 &           82.98 &  92.24 \\
     7 &    95.85 &        89.52 &           71.17 &  82.49 \\
     8 &    95.78 &        90.77 &           67.44 &  78.86 \\
     9 &    95.45 &        91.36 &           61.46 &  73.00 \\
    10 &    94.35 &        86.50 &           49.52 &  57.54 \\
    11 &    93.78 &        86.30 &           47.25 &  45.31 \\
    12 &    93.90 &        84.94 &           45.95 &  53.68 \\
    13 &    92.34 &          NaN &             NaN &    NaN \\
\bottomrule
\end{tabular}
}
\caption{Tagging and LM accuracies based on the last layer, after removal of TAG info in specific layers.
\ye{Need to work on this table. but the current columns are:}
probing: the probing performance of each layer (with no removal whatsoever).
rand dir lm: the performance of the task of interest from the last layer, after removing a random direction from layer i.
task: the performance of the task after removing a property from layer i.
P lm: the performance of the lm after removing property from layer i.}
\label{tbl:tag_lm_layers}

\end{table}


==> tables/layer_tag_removal.tex <==

\begin{table*}[ht]
\resizebox{\textwidth}{!}{%
% \begin{tabular}{c|ccccccccccccc}

% , & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13\\
% 1   & 30.66 & 74.43 & 78.29 & 82.67 & 83.62 & 85.65 & 85.72 & 85.37 & 84.57 & 84.29 & 82.99 & 79.83 & 76.67\\
% 2   & -  & 30.66 & 71.45 & 78.22 & 81.06 & 83.23 & 83.94 & 84.46 & 83.73 & 82.99 & 82.18 & 80.18 & 75.90\\
% 3   & -  & -  & 28.69 & 73.73 & 78.53 & 82.18 & 83.16 & 83.41 & 82.74 & 82.46 & 81.13 & 78.08 & 74.25\\
% 4   & -  & -  & -  & 26.34 & 75.03 & 74.68 & 78.01 & 81.23 & 81.80 & 81.13 & 80.01 & 75.73 & 71.34\\
% 5   & -  & -  & -  & -  & 25.01 & 69.48 & 74.01 & 76.75 & 77.03 & 75.41 & 74.39 & 72.04 & 65.98\\
% 6   & -  & -  & -  & -  & -  & 23.64 & 69.73 & 73.45 & 73.38 & 73.73 & 74.01 & 69.80 & 63.56\\
% 7   & -  & -  & -  & -  & -  & -  & 25.11 & 64.36 & 63.84 & 63.59 & 64.61 & 64.05 & 58.65\\
% 8   & -  & -  & -  & -  & -  & -  & -  & 23.71 & 55.49 & 59.91 & 58.72 & 57.31 & 54.54\\
% 9   & -  & -  & -  & -  & -  & -  & -  & -  & 25.18 & 47.18 & 48.75 & 48.54 & 43.32\\
% 10   & -  & -  & -  & -  & -  & -  & -  & -  & -  & 24.06 & 40.93 & 39.21 & 37.29\\
% 11   & -  & -  & -  & -  & -  & -  & -  & -  & -  & -  & 27.36 & 35.32 & 31.85\\
% 12   & -  & -  & -  & -  & -  & -  & -  & -  & -  & -  & -  & 23.85 & 33.46\\
% 13   & -  & -  & -  & -  & -  & -  & -  & -  & -  & -  & -  & 23.85 & 31.29\\

\begin{tabular}{llllllllllllllr}
\toprule
{} &  0 &        1 &        2 &        3 &        4 &        5 &        6 &        7 &        8 &        9 &       10 &       11 &       12 &     13 \\
\midrule
0  &  - &  85.17 &  86.37 &  87.89 &   89.5 &  89.72 &  90.29 &  90.13 &  89.84 &  89.28 &  88.57 &  86.67 &  87.29 &  83.28 \\
1  &  - &      - &  88.44 &  91.19 &  92.53 &  93.19 &  93.76 &  93.91 &  94.12 &  93.75 &  92.67 &  91.61 &  92.04 &  90.02 \\
2  &  - &      - &      - &  89.37 &  92.39 &  93.29 &  93.56 &  93.82 &  94.19 &  94.03 &  93.34 &  92.66 &  92.45 &  89.97 \\
3  &  - &      - &      - &      - &  90.22 &  91.78 &  92.68 &  93.25 &  92.85 &  92.88 &  91.67 &  90.81 &  90.09 &  88.45 \\
4  &  - &      - &      - &      - &      - &  88.99 &  90.81 &  91.72 &  92.12 &  91.92 &   91.2 &  89.92 &  89.51 &  86.47 \\
5  &  - &      - &      - &      - &      - &      - &  83.21 &  85.85 &  86.83 &  86.49 &   84.5 &  82.76 &  79.58 &  72.44 \\
6  &  - &      - &      - &      - &      - &      - &      - &  86.87 &  89.13 &  89.36 &  88.48 &  87.25 &  86.45 &  82.98 \\
7  &  - &      - &      - &      - &      - &      - &      - &      - &  79.21 &  79.09 &  79.16 &  78.11 &  77.27 &  71.17 \\
8  &  - &      - &      - &      - &      - &      - &      - &      - &      - &  76.42 &  74.53 &  75.05 &  74.46 &  67.44 \\
9  &  - &      - &      - &      - &      - &      - &      - &      - &      - &      - &  67.41 &  66.86 &  68.19 &  61.46 \\
10 &  - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &  56.69 &  55.94 &  49.52 \\
11 &  - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &  52.65 &  47.25 \\
12 &  - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &      - &  45.95 \\ \midrule
- & 83.65 & 92.81 & 94.16 & 95.09 & 95.88 & 95.91 & 95.9 & 95.85 & 95.78 & 95.45 & 94.35 & 93.78 & 93.9 & 92.34 \\
\bottomrule
\end{tabular}

% \end{tabular}

}
\caption{Tag accuracy when removing layer i (the rows) and test on layer j (columns). Tag. unmasked}
\label{tbl:layer_tag_deprobe}

\end{table*}

